Go Forth and Prosper: Language Modeling with Ancient Textual History

We introduce a technique for improving document-level language models (LM) by leveraging "ancient history": text that is outside the LM's current context window. We learn an auxiliary function to select spans from the ancient history which can help the LM to predict future text. The selected text spans are then copied directly into the LM's context window, replacing less predictive spans. This method can improve perplexity of pretrained LMs with no updates to the LM's own parameters. We further observe that an auxiliary function trained in a specific textual domain like Wikipedia will also work in a substantially different domain such as scientific publications. With this technique we see a 7 percent perplexity reduction on Wikipedia articles, and a 12 percent perplexity reduction on scientific texts.

==> method-backup.tex <==
Theoretically, an LM calculates the probability of a text $\mathcal{D} = {w_0 \ldots w_n}$ by factorizing the intractable distribution $P(\mathcal{D}|\theta)$ for model parameters $\theta$ as the conditional probability $\prod_{t \leq n} P(w_t|w_0 \ldots w_{t-1},\theta)$.\footnote{We omit $\theta$ hencefore for simplicity}
In practice, hardware limitations prohibit the complete factorization and LMs approximate the true distribution by conditioning at each timestep using just the $k$ most recent tokens i.e. $P(w_t|w_{t-k} \ldots w_{t-1})$.

This approximation is justified by the presumption that the last $k$ tokens contain enough information to predict $w_t$. 
What if this is not the case?
Especially when dealing with long documents, it's not obvious that the last $k$ tokens express much of the overall meaning of a document.

\begin{figure*}[ht]
\includegraphics[width=\textwidth]{acl-ijcnlp2021-templates/Overview.pdf}
\caption{Overview of Ancient History Language Modeling (Best Viewed in Color)}
\label{fig-overview}
\end{figure*}
 
Our technique effectively extends an LM's context to text beyond the last $k$ tokens and into the document's ancient history without needing to retrain the possibly inaccessible LM parameters. 
Figure~\ref{fig-overview} shows an overview of our approach. 
In traditional language modeling, the $k$ most recent tokens are fed to the LM. 
In our approach, we use the $j<k$ most recent tokens (called the ``necessary prefix'') to select $k-j$ additional tokens from the document's ancient history. 
This selection process uses an auxiliary selection function to identify spans from the ancient history that will help us predict future text. 
The training of this function is described below. 
Given a collection of spans selected by this function, we construct a new LM context window by concatenating the spans together with the necessary prefix. 
This new context is then fed to the LM to predict future text. 
Details of the inference process using this are given in Algorithm~\ref{alg-over}.

\begin{algorithm}[h]
\SetAlgoLined
\KwResult{Perplexity of LM on tokens $w_k\ldots w_{k+s}$ from $D$ for stride $s$}
 $D' = \{\mathcal{S}_i | \mathcal{S}_i = w_i \ldots w_{i+h}\},  0<i+h<k$ 
 Pretrained LM$(\cdot)$ with context window size $k+s$\;
 Auxiliary Fn AUX$(\cdot )$ \;
 $l\longleftarrow 0$
 $prefix \longleftarrow w_{k-j}\ldots w+{k-1}$
 
%  \While{While $l<(j-j)$}{
  
  
%   \eIf{condition}{
%   instructions1\;
%   instructions2\;
%   }{
%   instructions3\;
%   }
%  }
 \caption{\rikcomment{TODO: Inference algorithm}}
 \label{alg-over}
\end{algorithm}

\paragraph{Training Selection Function}
We model the auxiliary selection function (AUX) as a neural network. 
This network is trained to predict which spans from the ancient history should be used given a necessary prefix to construct a context for the LM. 
Specifically, given a span $\mathcal{S}_i$ from the document history and necessary prefix $\mathcal{P} = w_(k-j)\ldots w_{k-1}$, we compute the {\it score} of $\mathcal{S}_i, \mathcal{P}$ in terms of the likelihood of future text $\mathcal{F} = w_k\ldots w_{k+s}$ for stride s. 
The score is represented as the ratio of the likelihood under LM of $\mathcal{F}$ with and without $\mathcal{S}_i$ as context:
\begin{equation}
    \textrm{Score}(\mathcal{S}_i,\mathcal{P}) = P(\mathcal{F}|\mathcal{P}) / P(\mathcal{F}|\mathcal{S}_i,\mathcal{P})
    \label{eq-score}
\end{equation}

Spans which score higher under this function provide more information about future text compared to the prefix alone. 
The AUX network is trained to regress this score with the following objective:
\begin{equation}
    \mathcal{L} = \textrm{MSE}(\textrm{AUX}(\mathcal{S}_i,\mathcal{P})-\textrm{Score}(\mathcal{S}_i,\mathcal{P}))
    \label{eq-loss}
\end{equation}

At inference, AUX is used to rank spans from the ancient history for inclusion in the LM context window. 

% We approximate the function in Equation~\ref{eq-score} using GPT2 to encode the span/prefix pair \nascomment{you totally lost me here}. 
% The selected history in NCLM then consists of the top-$k$ \nascomment{how many is $k$?  how do you deal with different span lengths?  is there a max length?  I have no idea what the computational cost of this method is, and whether that's a training time cost or an inference time cost} scoring spans under this approximation.\footnote{We also experimented with scoring spans conditioned on previous span selections but found the time/performance trade-off unsatisfactory.}

